Learning Molecular Representation in a Cell

Predicting drug efficacy and safety in vivo requires information on biological responses (e.g., cell morphology and gene expression) to small molecule perturbations. However, current molecular representation learning methods do not provide a comprehensive view of cell states under these perturbations and struggle to remove noise, hindering model generalization. We introduce the Information Alignment (InfoAlign) approach to learn molecular representations through the information bottleneck method in cells. We integrate molecules and cellular response data as nodes into a context graph, connecting them with weighted edges based on chemical, biological, and computational criteria. For each molecule in a training batch, InfoAlign optimizes the encoder's latent representation with a minimality objective to discard redundant structural information. A sufficiency objective decodes the representation to align with different feature spaces from the molecule's neighborhood in the context graph. We demonstrate that the proposed sufficiency objective for alignment is tighter than existing encoder-based contrastive methods. Empirically, we validate representations from InfoAlign in two downstream applications: molecular property prediction against up to 27 baseline methods across four datasets, plus zero-shot molecule-morphology matching.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/chembl_broad.tex <==
\begin{table*}[t]
    \caption{Results on \chembl~and~\broad. We report average AUC (Avg.), as well as the percentage of tasks achieving AUC above 80\%, 85\%, and 90\%. \textbf{Best} and \underline{second best} mean are \textbf{bold} and \underline{underline}, respectively.}
    \label{tab:chembl-broad}
    \renewcommand{\arraystretch}{0.98}
    \renewcommand{\tabcolsep}{1.2mm}
    \centering
    \begin{adjustbox}{width=0.92\linewidth}
    \begin{tabular}{lllll|llll}
        \toprule
        & \multicolumn{4}{c|}{\chembl~(AUC $\uparrow$)} & \multicolumn{4}{c}{\broad~(AUC $\uparrow$)} \\
        % & \multicolumn{4}{c|}{\# Molecule: 2,355; \# Task: 41} & \multicolumn{4}{c}{\# Molecule: 6,567; \# Task: 32} \\
        (\# Molecule / \# Task) & \multicolumn{4}{c|}{(2355 / 41)} & \multicolumn{4}{c}{(6567 / 32)} \\
        \cmidrule{2-9}
        Method & Avg. & > 80 \% & > 85 \% & > 90 \% & Avg. & > 80 \% & > 85 \% & > 90 \% \\
        \midrule
        Morgan FP & 76.8±2.2 & 48.8±3.9 & 34.6±6.3 & 21.9±5.7 & \underline{63.3}±0.3 & 6.3±0.0 & \textbf{4.4}±1.7 & \textbf{3.1}±0.0 \\
        Pretrained GNN & 77.0±0.5 & 55.1±1.3 & 34.2±4.6 & 14.6±1.7 & 59.9±0.2 & \underline{7.5}±1.7 & \underline{3.1}±0.0 & \textbf{3.1}±0.0 \\
        Pretrained ChemLM & 74.7±1.9 & 46.3±3.4 & 35.1±4.4 & 22.9±1.3 & 60.6±0.3 & \underline{7.5}±1.7 & \underline{3.1}±0.0 & \underline{1.9}±1.7 \\
        Cell Morphology & 64.3±2.4 & 15.6±6.6 & 8.3±3.7 & 4.9±3.9 & 55.3±0.1 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
        Gene Expression & 56.1±1.1 & 5.1±1.4 & 3.4±1.3 & 3.4±1.3 & 56.9±1.4 & 1.9±1.7 & 1.9±1.7 & \underline{1.9}±1.7 \\
        \midrule
        CLOOME & 66.7±1.8 & 26.8±4.6 & 16.1±3.7 & 10.7±5.1 & 61.7±0.4 & 3.1±0.0 & \underline{3.1}±0.0 & 0.0±0.0 \\
        InfoCORE (GE) & \underline{79.3}±0.9 & \underline{62.4±}2.8 & \underline{46.3}±3.0 & \underline{30.3}±2.2 & 60.2±0.2 & 3.1±0.0 & 0.0±0.0 & 0.0±0.0 \\
        InfoCORE (CP) & 73.8±2.0 & 37.6±9.2 & 26.3±4.7 & 10.7±4.1 & 61.1±0.2 & 6.3±0.0 & \underline{3.1}±0.0 & 0.0±0.0 \\
        InfoAlign (Ours) & \textbf{81.3}±0.6 & \textbf{66.3}±2.7 & \textbf{49.3}±2.7 & \textbf{35.1}±3.7 & \textbf{70.0}±0.1 & \textbf{18.8}±2.2 & \underline{3.1}±0.0 & \textbf{3.1}±0.0 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}

==> tables/chembl_broad_merge.tex <==
\begin{table*}[t]
    \caption{Results on \chembl~(top) and \broad~(bottom): Left tables display average AUC (Avg.), as well as the percentage of tasks achieving AUC above 80\%, 85\%, and 90\%. Right figures show the distribution of performance across tasks.}
    \label{tab:chembl-broad}
    \centering

    % First set: \chembl
    \begin{minipage}{0.65\textwidth}
        \centering
        \begin{adjustbox}{width=\linewidth}
            \begin{tabular}{lllll}
                \toprule
                & \multicolumn{4}{c}{\chembl~(AUC $\uparrow$)} \\
                (\# Molecule, \# Task) & \multicolumn{4}{c}{(2,355, 41)} \\
                \cmidrule{2-5}
                Method & Avg. & > 80 \% & > 85 \% & > 90 \% \\
                \midrule
                Morgan FP & 76.8±2.2 & 48.8±3.9 & 34.6±6.3 & 21.9±5.7 \\
                Pretrained GNN & 77.0±0.5 & 55.1±1.3 & 34.2±4.6 & 14.6±1.7 \\
                Pretrained ChemLM & 74.7±1.9 & 46.3±3.4 & 35.1±4.4 & 22.9±1.3 \\
                Cell Morphology & 64.3±2.4 & 15.6±6.6 & 8.3±3.7 & 4.9±3.9 \\
                Gene Expression & 56.1±1.1 & 5.1±1.4 & 3.4±1.3 & 3.4±1.3 \\
                \midrule
                CLOOME & 66.7±1.8 & 26.8±4.6 & 16.1±3.7 & 10.7±5.1 \\
                InfoCORE (GE) & \underline{79.3}±0.9 & \underline{62.4}±2.8 & \underline{46.3}±3.0 & \underline{30.3}±2.2 \\
                InfoCORE (CP) & 73.8±2.0 & 37.6±9.2 & 26.3±4.7 & 10.7±4.1 \\
                InfoAlign (Ours) & \textbf{81.3}±0.6 & \textbf{66.3}±2.7 & \textbf{49.3}±2.7 & \textbf{35.1}±3.7 \\
                \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{minipage}%
    \begin{minipage}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/chembl2k_bar.pdf}
        \caption{\chembl~with 41 Tasks.} % Optional; add if needed
    \end{minipage}

    % Second set: \broad
    \begin{minipage}{0.65\textwidth}
        \centering
        \begin{adjustbox}{width=\linewidth}
            \begin{tabular}{lllll}
                \toprule
                & \multicolumn{4}{c}{\broad~(AUC $\uparrow$)} \\
                (\# Molecule, \# Task) & \multicolumn{4}{c}{(6,567, 32)} \\
                \cmidrule{2-5}
                Method & Avg. & > 80 \% & > 85 \% & > 90 \% \\
                \midrule
                Morgan FP & \underline{63.3}±0.3 & 6.3±0.0 & \textbf{4.4}±1.7 & \textbf{3.1}±0.0 \\
                Pretrained GNN & 59.9±0.2 & \underline{7.5}±1.7 & \underline{3.1}±0.0 & \textbf{3.1}±0.0 \\
                Pretrained ChemLM & 60.6±0.3 & \underline{7.5}±1.7 & \underline{3.1}±0.0 & \underline{1.9}±1.7 \\
                Cell Morphology & 55.3±0.1 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
                Gene Expression & 56.9±1.4 & 1.9±1.7 & 1.9±1.7 & \underline{1.9}±1.7 \\
                \midrule
                CLOOME & 61.7±0.4 & 3.1±0.0 & \underline{3.1}±0.0 & 0.0±0.0 \\
                InfoCORE (GE) & 60.2±0.2 & 3.1±0.0 & 0.0±0.0 & 0.0±0.0 \\
                InfoCORE (CP) & 61.1±0.2 & 6.3±0.0 & \underline{3.1}±0.0 & 0.0±0.0 \\
                InfoAlign (Ours) & \textbf{70.0}±0.1 & \textbf{18.8}±2.2 & \underline{3.1}±0.0 & \textbf{3.1}±0.0 \\
                \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{minipage}%
    \begin{minipage}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/broad6k_bar.pdf}
        \caption{\broad~with 32 Tasks.} % Optional; add if needed
    \end{minipage}
\end{table*}


==> tables/complete_broad6k.tex <==
\begin{table*}[t]
    \caption{Complete results on \broad. We report average AUC (Avg.), as well as the percentage of tasks achieving AUC above 80\%, 85\%, 90\% and 95\%. The best results in each category are {\sethlcolor{LightCyan}\hl{highlighted}} and reported in \cref{tab:chembl-broad}.}
    \label{tab:complete-broad}
    \renewcommand{\arraystretch}{0.95}
    \renewcommand{\tabcolsep}{1.2mm}
    \centering
    \begin{adjustbox}{width=0.85\linewidth}
    \begin{tabular}{lllllll}
    \toprule
    Repr. & Model &  Avg.  &  > 80 \% & > 85 \%  & > 90 \% & > 95\% \\
    \midrule
    \rowcolor{LightCyan} \multirow{3}{*}{Morgan FP} & MLP & 63.3±0.3 & 6.3±0.0 & 4.4±1.7 & 3.1±0.0 & 3.1±0.0 \\
     & RF & 55.5±0.1 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     & GP & 50.6±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     \midrule
    & AttrMask & 59.8±0.2 & 3.1±0.0 & 3.1±0.0 & 3.1±0.0 & 0.0±0.0 \\
     \rowcolor{LightCyan} Pretrained GNN & ContextPred & 60.0±0.2 & 7.5±1.7 & 3.1±0.0 & 3.1±0.0 & 0.0±0.0 \\
     & EdgePred & 59.9±0.2 & 3.1±0.0 & 3.1±0.0 & 3.1±0.0 & 0.0±0.0 \\
     \midrule
    % \multirow{4}{*}{Pretrained ChemLM} 
    & Roberta-102M & 59.8±0.7 & 5.0±1.7 & 3.1±0.0 & 3.1±0.0 & 0.0±0.0 \\
     \rowcolor{LightCyan} \multirow{2}{*}{Pretrained ChemLM} & GPT2-87M & 60.6±0.3 & 7.5±1.7 & 3.1±0.0 & 1.9±1.7 & 0.0±0.0 \\
     & MolT5 & 56.4±0.8 & 3.8±1.4 & 2.5±1.4 & 2.5±1.4 & 0.0±0.0 \\
     & ChemGPT-19M & 55.1±0.9 & 3.1±0.0 & 3.1±0.0 & 1.3±1.7 & 0.0±0.0 \\
     \midrule
    % \multirow{3}{*}{Cell Morphology} 
     & MLP & 51.9±1.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     \rowcolor{LightCyan} Cell Morphology & RF & 55.3±0.1 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     & GP & 54.7±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     \midrule
    \rowcolor{LightCyan} \multirow{3}{*}{Gene Expression} 
    & MLP & 56.9±1.4 & 1.9±1.7 & 1.9±1.7 & 1.9±1.7 & 0.0±0.0 \\
     & RF & 55.2±0.2 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     & GP & 50.1±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     \midrule
     \multirow{4}{*}{Aligned} 
     & CLOOME & 61.7±0.5 & 3.1±0.0 & 3.1±0.0 & 0.0±0.0 & 0.0±0.0 \\
     & InfoCORE (GE) & 60.2±0.2 & 3.1±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     & InfoCORE (CP) & 61.1±0.2 & 6.3±0.0 & 3.1±0.0 & 0.0±0.0 & 0.0±0.0 \\
     & InfoAlign & 69.9±0.1 & 18.8±2.2 & 3.1±0.0 & 3.1±0.0 & 1.3±1.7 \\

     \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}


==> tables/complete_chembl.tex <==
\begin{table*}[t]
    \caption{Complete results on \chembl. We report average AUC (Avg.), as well as the percentage of tasks achieving AUC above 80\%, 85\%, 90\% and 95\%. The best results in each category are {\sethlcolor{LightCyan}\hl{highlighted}} and reported in \cref{tab:chembl-broad}.}
    \label{tab:complete-chembl}
    \renewcommand{\arraystretch}{0.95}
    \renewcommand{\tabcolsep}{1.2mm}
    \centering
    \begin{adjustbox}{width=0.95\linewidth}
    \begin{tabular}{lllllll}
    \toprule
    Repr. & Model &  Avg.  &  > 80 \% & > 85 \%  & > 90 \% & > 95\% \\
    \midrule
    \rowcolor{LightCyan} \multirow{3}{*}{Morgan FP} 
     &  MLP & 76.8±2.2 & 48.8±3.9 & 34.6±6.3 & 21.9±5.7 & 12.2±2.4 \\
     & RF & 54.7±0.7 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     & GP & 51.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     \midrule
    & AttrMask & 74.0±0.5 & 46.8±2.7 & 31.2±4.4 & 14.6±1.7 & 2.4±0.0 \\
    \rowcolor{LightCyan} Pretrained GNN & ContextPred & 77.0±0.5 & 55.1±1.3 & 34.2±4.6 & 14.6±1.7 & 1.5±1.3 \\
    & EdgePred & 75.6±0.5 & 54.1±4.0 & 34.6±7.2 & 12.2±2.4 & 6.3±1.3 \\
    \midrule
    \rowcolor{LightCyan}  \multirow{4}{*}{Pretrained ChemLM} 
    & Roberta-102M & 74.7±1.9 & 46.3±3.5 & 35.1±4.4 & 22.9±1.3 & 7.8±3.2 \\
     & GPT2-87M & 71.0±3.4 & 31.2±11.2 & 20.0±9.4 & 7.3±6.9 & 2.9±3.2 \\
     & MolT5 & 70.0±0.8 & 32.2±2.0 & 21.0±4.1 & 8.8±1.3 & 3.4±1.3 \\
     & ChemGPT-19M & 65.0±1.1 & 16.1±2.8 & 11.2±3.3 & 5.4±1.1 & 2.9±1.1 \\
     \midrule
    \rowcolor{LightCyan}  \multirow{3}{*}{Cell Morphology} 
    & MLP & 64.3±2.4 & 15.6±6.6 & 8.3±3.7 & 4.9±3.9 & 2.9±2.7 \\
     & RF & 55.9±0.7 & 3.9±1.3 & 3.9±1.3 & 2.4±0.0 & 2.4±0.0 \\
     & GP & 51.5±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     \midrule
    \rowcolor{LightCyan}  \multirow{3}{*}{Gene Expression} 
    & MLP & 56.1±1.1 & 5.1±1.4 & 3.4±1.3 & 3.4±1.3 & 2.4±0.0 \\
     & RF & 52.8±0.3 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 & 0.0±0.0 \\
     & GP & \multicolumn{5}{c}{Run out of time} \\
     \midrule
     \multirow{4}{*}{Aligned} 
     & CLOOME & 66.7±1.8 & 26.8±4.6 & 16.1±3.7 & 10.7±5.1 & 3.4±2.8 \\
     & InfoCORE (GE) & 79.3±0.9 & 62.4±2.8 & 46.3±3.0 & 30.3±2.2 & 18.1±1.3 \\
     & InfoCORE (CP) & 73.8±2.0 & 37.6±9.2 & 26.3±4.7 & 10.7±4.1 & 5.9±2.2 \\
     & InfoAlign & 81.3±0.6 & 66.3±2.7 & 49.3±2.7 & 35.1±3.7 & 18.5±2.8 \\
     \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}


==> tables/complete_tox_biogen.tex <==
\begin{table*}[t]
    \caption{Complete results on \toxcast. We report average AUC (Avg.), as well as the percentage of tasks achieving AUC above 80\%, 85\%, 90\% and 95\%. The best results in each category are {\sethlcolor{LightCyan}\hl{highlighted}} and reported in \cref{tab:tox-biogen}.}
    \label{tab:complete-toxcast}
    \renewcommand{\arraystretch}{0.95}
    \renewcommand{\tabcolsep}{1.2mm}
    \centering
    \begin{adjustbox}{width=0.85\linewidth}
    \begin{tabular}{lllllll}
    \toprule
    \multicolumn{1}{l}{Representation} & Models & Avg. & \textgreater 80 \% & \textgreater 85 \% & \textgreater 90 \% & \textgreater 95 \% \\
    \midrule
    \rowcolor{LightCyan} \multirow{3}{*}{Morgan FP} & MLP & 57.6±1.0 & 1.6±0.3 & 0.6±0.4 & 0.3±0.3 & 0.0±0.0 \\
    & RF & 52.3±0.1 & 0.2±0.1 & 0.1±0.1 & 0.0±0.1 & 0.0±0.0 \\
     & GP & \multicolumn{5}{c}{Run out of time} \\
     \midrule
    % \multirow{3}{*}{Pretrained GNN} 
    & AttrMask & 63.1±0.8 & 3.2±1.2 & 0.8±0.3 & 0.2±0.1 & 0.0±0.1 \\
     Pretrained GNN  & ContextPred & 63.0±0.6 & 3.3±1.3 & 0.4±0.4 & 0.0±0.0 & 0.0±0.0 \\
     \rowcolor{LightCyan} & EdgePred & 63.5±1.1 & 4.8±3.0 & 0.8±0.4 & 0.1±0.1 & 0.0±0.0 \\
     \midrule
    % \multirow{4}{*}{Pretrained ChemLM} 
    & Roberta-102M & 64.2±0.8 & 3.1±1.8 & 0.9±0.6 & 0.2±0.2 & 0.0±0.1 \\
     Pretrained ChemLM & GPT2-87M & 61.5±1.1 & 2.4±0.6 & 0.8±0.3 & 0.3±0.1 & 0.0±0.1 \\
    \rowcolor{LightCyan} & MolT5 & 64.7±0.9 & 3.6±1.1 & 1.1±0.3 & 0.4±0.2 & 0.0±0.1 \\
     & ChemGPT-19M & \multicolumn{5}{c}{Token Error} \\
     \midrule
    \multirow{4}{*}{Aligned} & CLOOME & 54.2±1.0 & 0.9±0.2 & 0.3±0.1 & 0.1±0.1 & 0.0±0.0 \\
     & InfoCORE (GE) & 65.3±0.2 & 5.4±1.7 & 1.2±0.4 & 0.3±0.1 & 0.0±0.0 \\
     & InfoCORE (CP) & 62.4±0.4 & 1.3±0.5 & 0.3±0.3 & 0.0±0.0 & 0.0±0.0 \\
     & InfoAlign & 66.4±1.1 & 6.6±1.6 & 2.1±0.5 & 0.7±0.3 & 0.1±0.1 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}

\begin{table*}[t]
    \caption{Complete results on \biogen. We report the average MAE and MAE for all tasks (scaled by $\times$ 100). The best results in each category are {\sethlcolor{LightCyan}\hl{highlighted}} and reported in \cref{tab:tox-biogen}.}
    \label{tab:complete-biogen}
    \renewcommand{\arraystretch}{0.95}
    \renewcommand{\tabcolsep}{1.2mm}
    \centering
    \begin{adjustbox}{width=1\linewidth}
    \begin{tabular}{lllllllll}
    \toprule
    \multicolumn{1}{l}{Representation} & Models & Avg. & hPPB & rPPB & RLM & HLM & ER & Solubility \\
    \midrule
    % \multirow{3}{*}{Morgan FP} 
    & MLP & 66.2±2.4 & 66.1±2.6 & 56.8±2.3 & 56.5±4.2 & 74.6±6.2 & 73.7±7.3 & 69.5±3.0 \\
     \rowcolor{LightCyan} Morgan FP & RF & 52.8±0.2 & 44.2±0.1 & 44.2±0.1 & 41.9±0.2 & 67.7±0.7 & 66.9±0.9 & 51.6±0.1 \\
     & GP & 60.0±0.0 & 51.3±0.0 & 59.5±0.0 & 49.7±0.0 & 68.8±0.0 & 69.3±0.0 & 61.6±0.0 \\
     \midrule
    \rowcolor{LightCyan} \multirow{3}{*}{Pretrained GNN} 
    & AttrMask & 67.3±0.3 & 82.4±1.1 & 49.8±0.7 & 51.7±1.0 & 57.9±0.6 & 62.6±0.5 & 99.1±1.2 \\
     & ContextPred & 68.5±0.9 & 85.0±7.9 & 49.7±0.4 & 55.1±2.7 & 61.4±1.8 & 63.1±0.5 & 96.5±3.7 \\
     & EdgePred & 67.8±0.9 & 81.2±10.2 & 48.0±0.5 & 53.5±2.8 & 62.2±1.8 & 62.9±0.7 & 99.1±6.9 \\
     \midrule
    % \multirow{4}{*}{Pretrained ChemLM} 
    & Roberta-102M & 69.0±2.6 & 71.4±14.5 & 65.1±19.2 & 63.7±24.6 & 67.5±5.2 & 69.9±4.9 & 76.7±13.2 \\
     Pretrained ChemLM & GPT2-87M & 73.9±8.5 & 65.4±12.9 & 73.1±20.8 & 54.1±12.9 & 83.2±21.5 & 86.1±19.8 & 81.8±25.5 \\
     \rowcolor{LightCyan} & MolT5 & 65.1±0.5 & 76.7±2.1 & 55.9±1.1 & 49.2±1.0 & 70.3±0.8 & 73.1±1.0 & 65.3±1.7 \\
     & ChemGPT-19M & 75.7±8.5 & 59.5±7.3 & 88.8±32.3 & 76.1±11.8 & 84.0±20.6 & 77.2±8.5 & 68.6±7.1 \\
     \midrule
    \multirow{4}{*}{Aligned} & CLOOME & 64.3±0.4 & 65.2±1.5 & 56.9±0.8 & 44.2±0.8 & 70.7±0.4 & 73.6±0.8 & 75.0±2.1 \\
     & InfoCORE (GE) & 69.9±1.2 & 79.9±3.6 & 51.6±1.8 & 51.3±2.1 & 78.6±0.3 & 77.8±1.9 & 80.4±0.9 \\
     & InfoCORE (CP) & 71.0±0.6 & 74.5±4.9 & 53.5±0.7 & 53.6±2.1 & 80.8±1.5 & 79.4±3.4 & 84.4±1.0 \\
     & InfoAlign & 49.4±0.2 & 39.7±0.4 & 39.2±0.3 & 40.5±0.6 & 66.7±1.7 & 62.0±1.5 & 48.4±0.6 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}


==> tables/tox_biogen.tex <==
\begin{table*}[t]
    \caption{Results on \toxcast~and~\biogen. We report the average AUC and the percentage of AUC above 80\% on \toxcast, and regression MAE (scaled by × 100) for \biogen. \textbf{Best} and \underline{second best} mean are \textbf{bold} and \underline{underline}, respectively.}
    \label{tab:tox-biogen}
    \renewcommand{\arraystretch}{0.9}
    \renewcommand{\tabcolsep}{0.8mm}
    \centering
    \begin{adjustbox}{width=1.01\linewidth}
    \begin{tabular}{lll|lllllll}
    \toprule
    & \multicolumn{2}{c|}{\toxcast~(AUC $\uparrow$)} & \multicolumn{7}{c}{\biogen~(MAE $\times 100 \downarrow$ )} \\
    (\# Molecule / \# Task) & \multicolumn{2}{c|}{(8576 / 617)} & \multicolumn{7}{c}{(3521 / 6)} \\
    \cmidrule{2-10}
    Method & Avg. & \textgreater 80 \% & Avg. & hPPB & rPPB & RLM & HLM & ER & Solubility \\
    % MDCK-MDR1 ER
    \midrule
    Morgan FP & 57.6±1.0 & 1.6±0.3 & \underline{52.8}±0.2 & \underline{44.2}±0.1 & \underline{44.2}±0.1 & \underline{42.0}±0.2 & 67.7±0.7 & 66.9±0.9 & \underline{51.6}±0.1 \\
    Pretrained GNN & 63.5±1.1 & 4.8±3.0 & 67.3±0.3 & 82.4±1.1 & 49.8±0.7 & 51.7±1.0 & \textbf{57.9}±0.6 & \underline{62.6}±0.5 & 99.1±1.2 \\
    Pretrained ChemLM & 64.7±0.9 & 3.6±1.1 & 65.1±0.5 & 76.7±2.1 & 55.9±1.1 & 49.2±1.0 & 70.3±0.8 & 73.1±1.0 & 65.3±1.7 \\
    \midrule
    CLOOME & 54.2±0.9 & 0.9±0.2 & 64.3±0.4 & 65.2±1.5 & 56.9±0.8 & 44.2±0.8 & 70.7±0.4 & 73.6±0.8 & 75.0±2.1 \\
    InfoCORE (GE) & \underline{65.3}±0.2 & \underline{5.4}±1.7 & 69.9±1.2 & 79.9±3.6 & 51.6±1.8 & 51.3±2.1 & 78.6±0.3 & 77.8±1.9 & 80.3±0.9 \\
    InfoCORE (CP) & 62.4±0.4 & 1.3±0.5 & 71.0±0.6 & 74.5±4.9 & 53.5±0.7 & 53.6±2.1 & 80.8±1.5 & 79.4±3.4 & 84.4±1.0 \\
    InfoAlign (Ours) & \textbf{66.4}±1.1 & \textbf{6.6}±1.6 & \textbf{49.4}±0.2 & \textbf{39.7}±0.4 & \textbf{39.2±}0.3 & \textbf{40.5}±0.6 & \underline{66.7}±1.7 & \textbf{62.0}±1.5 & \textbf{48.4}±0.6 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}

